Combining time-dependent density functional theory and the $\Delta$SCF approach for accurate core-electron spectra

Spectroscopies that probe electronic excitations from core levels into unoccupied orbitals, such as X-ray absorption spectroscopy and electron energy loss spectroscopy, are widely used to gain insight into the electronic and chemical structure of materials. To support the interpretation of experimental spectra, we assess the performance of a first-principles approach that combines linear-response time-dependent density (TDDFT) functional theory with the $\Delta$~self\nobreakdash-consistent field ($\Delta$SCF) approach. In particular, we first use TDDFT to calculate the core-level spectrum and then shift the spectrum such that the lowest excitation energy from TDDFT agrees with that from $\Delta$SCF. We apply this method to several small molecules and find encouraging agreement between calculated and measured spectra.

==> table_dumps/Updated_tables/IP_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Theoretical core IP results vs experiment
}
\label{IP_full}
%\resizebox{\p}{!}
{
\begin{tabular}{|l|l|r|c|r|c|c|c|c|}
\hline
\tiny
Species & Target Atom & Experiment & B3LYP & BHLYP & BLYP & PBE0 & PBE & SCAN \\ \hline
CH3 & C & 290.7 & 290.7 & 290.6 & 290.6 & 290.5 & 290.7 & 290.7 \\ \hline
NH3 & N & 405.6 & 405.6 & 405.9 & 405.6 & 405.7 & 405.5 & 405.5 \\ \hline
H2O & O & 539.7 & 539.7 & 539.5 & 539.4 & 539.5 & 539.6 & 539.6 \\ \hline
HF & F & 694.1 & 694.2 & 694.4 & 694.2 & 694.5 & 694.1 & 694.1 \\ \hline
OCS & C & 295.2 & 295.3 & 295.3 & 295.1 & 295.0 & 295.0 & 295.0 \\ \hline
 & O & 540.3 & \multicolumn{1}{r|}{540.2} & 540.6 & \multicolumn{1}{r|}{540.1} & \multicolumn{1}{r|}{539.6} & \multicolumn{1}{r|}{539.3} & \multicolumn{1}{r|}{540.3} \\ \hline
CO & C & 296.2 & 296.7 & 296.3 & 296.5 & 295.5 & 295.7 & 296.5 \\ \hline
 & O & 542.1 & 542.4 & 542.4 & 542.6 & 541.7 & 541.7 & 542.6 \\ \hline
Acetone & C(H3) & 291.2 & 291.2 & 291.4 & 291.5 & 291.9 & 291.8 & 291.4 \\ \hline
 & C(O) & 293.9 & 293.8 & 293.9 & 293.9 & 294.0 & 294.1 & 294.1 \\ \hline
 & O & 537.9 & \multicolumn{1}{r|}{537.5} & 537.8 & \multicolumn{1}{r|}{537.5} & \multicolumn{1}{r|}{537.0} & \multicolumn{1}{r|}{536.7} & \multicolumn{1}{r|}{537.6} \\ \hline
C2H4 & C & 290.6 & 290.9 & 290.8 & 290.9 & 291.3 & 291.0 & 290.8 \\ \hline
C2H2 & C & 291.2 & 291.4 & 291.5 & 291.7 & 291.8 & 291.6 & 291.3 \\ \hline
Formaldehyde & C & 294.5 & 294.5 & 294.6 & 294.8 & 294.8 & 294.7 & \multicolumn{1}{r|}{294.5} \\ \hline
 &  & 539.0 & 539.3 & 539.5 & 539.7 & 539.7 & 539.8 & \multicolumn{1}{r|}{539.3} \\ \hline
Ethanol & C(H2OH) & 291.1 & 290.9 & 291.1 & 291.3 & 291.3 & 291.4 & 290.9 \\ \hline
 & C(H3­) & 292.5 & 292.1 & 292.5 & 292.6 & 292.8 & 292.6 & 292.4 \\ \hline
 & O & 538.6 & 538.2 & 539.0 & \multicolumn{1}{r|}{538.6} & \multicolumn{1}{r|}{538.1} & \multicolumn{1}{r|}{537.9} & \multicolumn{1}{r|}{538.6} \\ \hline
Pyridine & C & -- & -- & -- & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & -- \\ \hline
- & N & 404.9 & 404.5 & 404.8 & 404.9 & 405.2 & 405.2 & 404.6 \\ \hline
Pyridazine & C & -- & -- & -- & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & -- \\ \hline
 & N & 404.9 & 405.2 & 405.2 & 405.3 & 405.3 & 405.3 & 404.7 \\ \hline
Pyrimidine & C & -- & -- & -- & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & \multicolumn{1}{l|}{--} & -- \\ \hline
 & N & 405.2 & 404.6 & 405.3 & 405.5 & 405.7 & 405.8 & 405.0 \\ \hline
Pyrazine & C & 291.7 & 291.4 & 291.4 & 291.6 & 291.7 & 291.6 & 291.5 \\ \hline
 & N & 405.6 & 405.2 & 405.5 & 405.6 & 406.2 & 406.6 & 405.6 \\ \hline
\textbf{Abs Mean error} & -- & -- & \multicolumn{1}{r|}{0.236} & 0.188 & \multicolumn{1}{r|}{0.228} & \multicolumn{1}{r|}{0.422} & \multicolumn{1}{r|}{0.418} & \multicolumn{1}{r|}{0.163} \\ \hline
\textbf{Mean error *} & -- & -- & \multicolumn{1}{r|}{-0.1} & 0.1 & \multicolumn{1}{r|}{0.1} & \multicolumn{1}{r|}{0.1} & \multicolumn{1}{r|}{0.0} & \multicolumn{1}{r|}{0.0} \\ \hline
\end{tabular}%
}
\end{table}

==> table_dumps/Updated_tables/K_edge_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Theoretical K-edge results vs experiment
}
\label{K_edge_full}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c |}
\hline
{\color[HTML]{333333} Species} & {\color[HTML]{333333} Target Atom} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} Experiment}} & {\color[HTML]{333333} B3LYP} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} BHLYP}} & {\color[HTML]{333333} BLYP} & {\color[HTML]{333333} PBE0} & {\color[HTML]{333333} PBE} & {\color[HTML]{333333} SCAN} \\ \hline
{\color[HTML]{333333} CH3} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 286.8} & {\color[HTML]{333333} 286.4} & {\color[HTML]{333333} 286.5} & {\color[HTML]{333333} 286.6} & {\color[HTML]{333333} 286.7} & {\color[HTML]{333333} 286.8} & {\color[HTML]{333333} 286.4} \\ \hline
{\color[HTML]{333333} NH3} & {\color[HTML]{333333} N} & {\color[HTML]{333333} 400.4} & {\color[HTML]{333333} 399.9} & {\color[HTML]{333333} 400.4} & {\color[HTML]{333333} 400.5} & {\color[HTML]{333333} 400.6} & {\color[HTML]{333333} 400.6} & {\color[HTML]{333333} 400.5} \\ \hline
{\color[HTML]{333333} H2O} & {\color[HTML]{333333} O} & {\color[HTML]{333333} 533.9} & {\color[HTML]{333333} 534.5} & {\color[HTML]{333333} 534.2} & {\color[HTML]{333333} 534.2} & {\color[HTML]{333333} 534.6} & {\color[HTML]{333333} 534.7} & {\color[HTML]{333333} 534.2} \\ \hline
{\color[HTML]{333333} HF} & {\color[HTML]{333333} F} & {\color[HTML]{333333} 687.3} & {\color[HTML]{333333} 687.4} & {\color[HTML]{333333} 687.4} & {\color[HTML]{333333} 687.6} & {\color[HTML]{333333} 687.7} & {\color[HTML]{333333} 687.7} & {\color[HTML]{333333} 687.4} \\ \hline
{\color[HTML]{333333} OCS} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 288.4} & {\color[HTML]{333333} 287.6} & {\color[HTML]{333333} 287.6} & {\color[HTML]{333333} 287.6} & {\color[HTML]{333333} 287.8} & {\color[HTML]{333333} 287.7} & {\color[HTML]{333333} 287.8} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} O} & {\color[HTML]{333333} 533.1} & {\color[HTML]{333333} 533.3} & {\color[HTML]{333333} 533.2} & {\color[HTML]{333333} 533.5} & {\color[HTML]{333333} 532.8} & {\color[HTML]{333333} 532.7} & {\color[HTML]{333333} 533.5} \\ \hline
{\color[HTML]{333333} CO} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 287.3} & {\color[HTML]{333333} 287.4} & {\color[HTML]{333333} 287.2} & {\color[HTML]{333333} 287.3} & {\color[HTML]{333333} 287.4} & {\color[HTML]{333333} 287.4} & {\color[HTML]{333333} 286.4} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} O} & {\color[HTML]{333333} 533.1} & {\color[HTML]{333333} 533.6} & {\color[HTML]{333333} 533.3} & {\color[HTML]{333333} 533.5} & {\color[HTML]{333333} 533.9} & {\color[HTML]{333333} 534.0} & {\color[HTML]{333333} 533.8} \\ \hline
{\color[HTML]{333333} Acetone} & {\color[HTML]{333333} C(H3)} & {\color[HTML]{333333} 286.4} & {\color[HTML]{333333} 286.8} & {\color[HTML]{333333} 286.8} & {\color[HTML]{333333} 286.9} & {\color[HTML]{333333} 287.0} & {\color[HTML]{333333} 287.0} & {\color[HTML]{333333} 286.8} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} C(O)} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} O} & {\color[HTML]{333333} 530.7} & {\color[HTML]{333333} 530.6} & {\color[HTML]{333333} 531.0} & {\color[HTML]{333333} 531.0} & {\color[HTML]{333333} 530.1} & {\color[HTML]{333333} 530.2} & {\color[HTML]{333333} 530.7} \\ \hline
{\color[HTML]{333333} C2H4} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 284.4} & {\color[HTML]{333333} 284.2} & {\color[HTML]{333333} 284.3} & {\color[HTML]{333333} 284.3} & {\color[HTML]{333333} 284.3} & {\color[HTML]{333333} 284.4} & {\color[HTML]{333333} 284.2} \\ \hline
{\color[HTML]{333333} C2H2} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 285.6} & {\color[HTML]{333333} 285.6} & {\color[HTML]{333333} 285.1} & {\color[HTML]{333333} 286.0} & {\color[HTML]{333333} 285.8} & {\color[HTML]{333333} 285.4} & {\color[HTML]{333333} 285.1} \\ \hline
{\color[HTML]{333333} Formaldehyde} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 285.6} & {\color[HTML]{333333} 285.4} & {\color[HTML]{333333} 285.4} & {\color[HTML]{333333} 285.5} & {\color[HTML]{333333} 285.7} & {\color[HTML]{333333} 285.8} & {\color[HTML]{333333} 285.4} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} --} & {\color[HTML]{333333} 530.8} & {\color[HTML]{333333} 530.6} & {\color[HTML]{333333} 530.6} & {\color[HTML]{333333} 530.7} & {\color[HTML]{333333} 530.8} & {\color[HTML]{333333} 530.8} & {\color[HTML]{333333} 530.6} \\ \hline
{\color[HTML]{333333} Ethanol} & {\color[HTML]{333333} C(H2OH)} & {\color[HTML]{333333} 286.9} & {\color[HTML]{333333} 287.0} & {\color[HTML]{333333} 287.0} & {\color[HTML]{333333} 287.1} & {\color[HTML]{333333} 287.2} & {\color[HTML]{333333} 287.3} & {\color[HTML]{333333} 287.0} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} C(H3­)} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} O} & {\color[HTML]{333333} 532.6} & {\color[HTML]{333333} ***} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} ***}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 533.4}} & {\color[HTML]{333333} 533.6} & {\color[HTML]{333333} 534.1} & {\color[HTML]{333333} 533.6} \\ \hline
{\color[HTML]{333333} Pyridine} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 284.9} & {\color[HTML]{333333} 284.2} & {\color[HTML]{333333} 284.4} & {\color[HTML]{333333} 284.3} & {\color[HTML]{333333} 284.8} & {\color[HTML]{333333} 284.6} & {\color[HTML]{333333} 284.5} \\ \hline
{\color[HTML]{333333} -} & {\color[HTML]{333333} N} & {\color[HTML]{333333} 398.8} & {\color[HTML]{333333} 398.3} & {\color[HTML]{333333} 398.4} & {\color[HTML]{333333} 398.5} & {\color[HTML]{333333} 398.6} & {\color[HTML]{333333} 398.7} & {\color[HTML]{333333} 398.7} \\ \hline
{\color[HTML]{333333} Pyridazine} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 285.5} & {\color[HTML]{333333} 285.8} & {\color[HTML]{333333} 285.6} & {\color[HTML]{333333} 285.7} & {\color[HTML]{333333} 285.8} & {\color[HTML]{333333} 285.8} & {\color[HTML]{333333} 285.8} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} N} & {\color[HTML]{333333} 399.0} & {\color[HTML]{333333} 398.8} & {\color[HTML]{333333} 398.9} & {\color[HTML]{333333} 399.0} & {\color[HTML]{333333} 399.1} & {\color[HTML]{333333} 399.1} & {\color[HTML]{333333} 399.1} \\ \hline
{\color[HTML]{333333} Pyrimidine} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 284.9} & {\color[HTML]{333333} 285.0} & {\color[HTML]{333333} 285.1} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.7} & {\color[HTML]{333333} 285.1} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} N} & {\color[HTML]{333333} 398.8} & {\color[HTML]{333333} 398.2} & {\color[HTML]{333333} 398.3} & {\color[HTML]{333333} 398.4} & {\color[HTML]{333333} 398.4} & {\color[HTML]{333333} 398.5} & {\color[HTML]{333333} 398.5} \\ \hline
{\color[HTML]{333333} Pyrazine} & {\color[HTML]{333333} C} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.1} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.3} & {\color[HTML]{333333} 285.0} \\ \hline
{\color[HTML]{333333} } & {\color[HTML]{333333} N} & {\color[HTML]{333333} 398.8} & {\color[HTML]{333333} 399.0} & {\color[HTML]{333333} 399.1} & {\color[HTML]{333333} 399.3} & {\color[HTML]{333333} 399.8} & {\color[HTML]{333333} 399.4} & {\color[HTML]{333333} 399.0} \\ \hline
{\color[HTML]{333333} \textbf{Abs Mean error}} & {\color[HTML]{333333} --} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.313}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.254}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.309}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.358}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.392}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.334}} \\ \hline
{\color[HTML]{333333} \textbf{Mean error *}} & {\color[HTML]{333333} --} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} --}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} -0.1}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} -0.1}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.1}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.2}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.2}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 0.0}} \\ \hline
\end{tabular}%
}
\end{table}

==> table_dumps/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\centering
\caption{XC Performance per target element for Core IP}
\label{table3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Target Atom}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}No. Points} & {\color[HTML]{000000} \textit{B3LYP}} & {\color[HTML]{000000} \textit{BHLYP}} & {\color[HTML]{000000} \textit{BLYP}} & {\color[HTML]{000000} \textit{PBE0}} & {\color[HTML]{000000} \textit{PBE}} & {\color[HTML]{000000} \textit{SCAN}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}C} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}9} & {\color[HTML]{000000} 0.18} & {\color[HTML]{000000} 0.11} & {\color[HTML]{000000} 0.22} & {\color[HTML]{000000} 0.40} & {\color[HTML]{000000} 0.29} & {\color[HTML]{000000} 0.15} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}O} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}6} & {\color[HTML]{000000} 0.23} & {\color[HTML]{000000} 0.25} & {\color[HTML]{000000} 0.31} & {\color[HTML]{000000} 0.50} & {\color[HTML]{000000} 0.62} & {\color[HTML]{000000} 0.21} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}N} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}5} & {\color[HTML]{000000} 5.00} & {\color[HTML]{000000} 0.18} & {\color[HTML]{000000} 0.14} & {\color[HTML]{000000} 0.38} & {\color[HTML]{000000} 0.48} & {\color[HTML]{000000} 0.16} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} & {\color[HTML]{000000} 0.10} & {\color[HTML]{000000} 0.30} & {\color[HTML]{000000} 0.10} & {\color[HTML]{000000} 0.40} & {\color[HTML]{000000} 0.00} & {\color[HTML]{000000} 0.00} \\ \hline
\multicolumn{1}{l|}{Average} & \multicolumn{1}{l|}{21} & {\color[HTML]{000000} 0.24} & {\color[HTML]{000000} 0.19} & {\color[HTML]{000000} 0.23} & {\color[HTML]{000000} 0.42} & {\color[HTML]{000000} 0.42} & {\color[HTML]{000000} 0.16} \\ \hline
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} }
\end{tabular}%
}
\end{table}

==> table_dumps/table4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\centering
\caption{XC Performance per target element for K1 Edge}
\label{table4}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrr}
\hline
\multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Target Atom}} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}No. Points} & {\color[HTML]{000000} \textit{B3LYP}} & {\color[HTML]{000000} \textit{BHLYP}} & {\color[HTML]{000000} \textit{BLYP}} & {\color[HTML]{000000} \textit{PBE0}} & {\color[HTML]{000000} \textit{PBE}} & {\color[HTML]{000000} \textit{SCAN}} \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}C} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}11} & {\color[HTML]{000000} 0.29} & {\color[HTML]{000000} 0.28} & {\color[HTML]{000000} 0.29} & {\color[HTML]{000000} 0.24} & {\color[HTML]{000000} 0.30} & {\color[HTML]{000000} 0.38} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}O} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}5} & {\color[HTML]{000000} 0.32} & {\color[HTML]{000000} 0.23} & {\color[HTML]{000000} 0.30} & {\color[HTML]{000000} 0.48} & {\color[HTML]{000000} 0.52} & {\color[HTML]{000000} 0.32} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}N} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}5} & {\color[HTML]{000000} 0.40} & {\color[HTML]{000000} 0.26} & {\color[HTML]{000000} 0.26} & {\color[HTML]{000000} 0.38} & {\color[HTML]{000000} 0.26} & {\color[HTML]{000000} 0.16} \\
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}F} & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} & {\color[HTML]{000000} 0.10} & {\color[HTML]{000000} 0.10} & {\color[HTML]{000000} 0.30} & {\color[HTML]{000000} 0.40} & {\color[HTML]{000000} 0.40} & {\color[HTML]{000000} 0.10} \\ \hline
\multicolumn{1}{l|}{Average} & \multicolumn{1}{l|}{24} & {\color[HTML]{000000} 0.31} & {\color[HTML]{000000} 0.25} & {\color[HTML]{000000} 0.31} & {\color[HTML]{000000} 0.36} & {\color[HTML]{000000} 0.39} & {\color[HTML]{000000} 0.33} \\ \hline
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } \\
\cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} } & {\color[HTML]{000000} }
\end{tabular}%
}
\end{table}

==> table_dumps/table5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{Relative Time Performance of Functionals}
\label{table5}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll}
\cline{1-7}
\multicolumn{1}{l|}{Functional} & \multicolumn{1}{c}{\textit{B3LYP}} & \multicolumn{1}{c}{\textit{BHLYP}} & \multicolumn{1}{c}{\textit{BLYP}} & \multicolumn{1}{c}{\textit{PBE0}} & \multicolumn{1}{c}{\textit{PBE}} & \multicolumn{1}{c}{\textit{SCAN}} &  \\ \cline{1-7}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Relative Total \\ Time (s)\end{tabular}} & \multicolumn{1}{r}{5.4} & \multicolumn{1}{r}{5.7} & \multicolumn{1}{r}{1.0} & \multicolumn{1}{r}{5.8} & \multicolumn{1}{r}{1.1} & \multicolumn{1}{r}{2.1} &  \\ \cline{1-7}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Relative Time\\  per Iteration (s)\end{tabular}} & \multicolumn{1}{r}{4.2} & \multicolumn{1}{r}{4.1} & \multicolumn{1}{r}{1.0} & \multicolumn{1}{r}{4.1} & \multicolumn{1}{r}{1.0} & \multicolumn{1}{r}{1.5} &  \\ \cline{1-7}
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  & 
\end{tabular}%
}
\end{table}

==> table_dumps/td_dks_nh3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{Performance of TD-DFT vs DKS for the K1 edge of NH3}
\label{td_dks_nh3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcllllll}
\cline{1-5}
\multicolumn{1}{|l|}{TD-DFT Functional} & \multicolumn{1}{r}{\textit{BHLYP}} & \multicolumn{1}{r}{\textit{BLYP}} & \multicolumn{1}{r}{\textit{PBE0}} & \multicolumn{1}{r}{\textit{HF}} & \multicolumn{1}{r}{\textit{}} & \multicolumn{1}{r}{\textit{}} &  \\ \cline{1-5}
\multicolumn{1}{l|}{TD-DFT K1 Edge (eV)} & \multicolumn{1}{r}{398.7} & \multicolumn{1}{r}{379.9} & \multicolumn{1}{r}{389.1} & \multicolumn{1}{r}{416.0} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} &  \\ \cline{1-5}
\multicolumn{1}{l|}{Experimental K1 Edge (eV)} & \multicolumn{4}{c}{400.4} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} &  \\ \cline{1-5}
\multicolumn{1}{l|}{DKS Functional} & BHLYP & \multicolumn{1}{r}{\textit{BLYP}} & \multicolumn{1}{r}{\textit{PBE0}} & \textit{SCAN} &  &  &  \\ \cline{1-5}
\multicolumn{1}{l|}{DKS K1 Edge (eV)} & 400.4 & 400.5 & 400.6 & 400.5 &  &  &  \\ \cline{1-5}
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\
 &  &  &  &  &  &  &  \\ \hline
\end{tabular}%
}
\end{table}
